Search for rare $B^0_{(s)}\rightarrow \mu^+ \mu^- \mu^+ \mu^-$ decays

\noindent A search for the decays $B^0_{s}\rightarrow \mu^+ \mu^- \mu^+ \mu^-$ and $B^0 \rightarrow \mu^+ \mu^- \mu^+ \mu^-$ is performed using data, corresponding to an integrated luminosity of 1.0\ensuremath{\{\,fb}^{-1}}\xspace, collected with the LHCb detector in 2011. The number of candidates observed is consistent with the expected background and, assuming phase-space models of the decays, limits on the branching fractions are set: \{${\ensuremath{\cal B}\xspace}(B^0_{s}\rightarrow \mu^+ \mu^- \mu^+ \mu^-) < 1.6 \ (1.2) \times 10^{-8}$} and \{${\ensuremath{\cal B}\xspace}(B^0 \rightarrow \mu^+ \mu^- \mu^+ \mu^-)< 6.6 \ (5.3) \times 10^{-9}$} at 95\,% (90\,%) confidence level. In addition, limits are set in the context of a supersymmetric model which allows for the $B^0_{(s)}$ meson to decay into a scalar ($S$) and pseudoscalar particle ($P$), where $S$ and $P$ have masses of 2.5 GeV and 214.3 MeV, respectively, both resonances decay into $\mu^+\mu^-$. The branching fraction limits for these decays are \{${\ensuremath{\cal B}\xspace}(\ensuremath{B^0_{s}\rightarrow SP}\xspace) < 1.6 \ (1.2) \times 10^{-8}$} and \{${\ensuremath{\cal B}\xspace}(\ensuremath{B^0\rightarrow SP}\xspace)< 6.3 \ (5.1) \times 10^{-9}$} at 95% (90%) confidence level.

==> bibliography.tex <==
%\cleardoublepage

%\addcontentsline{toc}{chapter}{Bibliography}

%\baselineskip=3ex

%\newcommand{\BIBand}{\&}
\bibliographystyle{LHCb}

%\pagestyle{myheadings}
%\markboth{Bibliography}{Bibliography}

\bibliography{main}  

